A Solution toward Transparent and Practical AI Regulation: Privacy Nutrition Labels for Open-source Generative AI-based Applications

The rapid development and widespread adoption of Generative Artificial Intelligence-based (GAI) applications have greatly enriched our daily lives, benefiting people by enhancing creativity, personalizing experiences, improving accessibility, and fostering innovation and efficiency across various domains. However, along with the development of GAI applications, concerns have been raised about transparency in their privacy practices. Traditional privacy policies often fail to effectively communicate essential privacy information due to their complexity and length, and open-source community developers often neglect privacy practices even more. Only 12.2% of examined open-source GAI apps provide a privacy policy. To address this, we propose a regulation-driven GAI Privacy Label and introduce Repo2Label, a novel framework for automatically generating these labels based on code repositories. Our user study indicates a common endorsement of the proposed GAI privacy label format. Additionally, Repo2Label achieves a precision of 0.81, recall of 0.88, and F1-score of 0.84 based on the benchmark dataset, significantly outperforming the developer self-declared privacy notices. We also discuss the common regulatory (in)compliance of open-source GAI apps, comparison with other privacy notices, and broader impacts to different stakeholders. Our findings suggest that Repo2Label could serve as a significant tool for bolstering the privacy transparency of GAI apps and make them more practical and responsible.

==> table/avg_performance.tex <==
\begin{table*}
\centering
\caption{Average performance of Repo2Label framework. The Average* group is the result of not counting prompt tokens greater than 8000. The Average* group has a higher recall than the Average group.}
\begin{tabular}{ll|ccc|ccc}
 \toprule
 &  & \multicolumn{3}{c|}{\textbf{Average}} & \multicolumn{3}{c}{\textbf{Average*}} \\ \midrule
\textbf{LLM} & \textbf{Experiment Settings} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} \\ \midrule
GPT-4o & zero-shot & .68 & .84 & .75 & .68 & \textbf{.86} & .76 \\
 & zero-shot + verification & .81 & .88 & .84 & .82 & \textbf{.89} & .85 \\
 & few-shot & .67 & .83 & .74 & .67 & \textbf{.85} & .75 \\
 & few-shot + verification & .79 & .87 & .83 & .79 & \textbf{.88} & .83 \\ \midrule
GPT-4 Turbo & zero-shot & .64 & .68 & .66 & .65 & \textbf{.69} & .67 \\
 & zero-shot + verification & .65 & .68 & .66 & .65 & \textbf{.69} & .67 \\
 & few-shot & .58 & .71 & .64 & .58 & \textbf{.73} & .64 \\
 & few-shot + verification & .60 & .73 & .66 & .60 & \textbf{.75} & .66 \\ \midrule
\end{tabular}
\label{avg_performance}
\end{table*}

==> table/regulation-empirical_study.tex <==
\begin{table*}[h]
\footnotesize
% \small
\begin{tabular}{
  @{}
    >{\centering\arraybackslash}p{0.05\textwidth}
    >{\centering\arraybackslash}p{0.1\textwidth}
    >{\centering\arraybackslash}p{0.1\textwidth}|
    >{\centering\arraybackslash}p{0.25\textwidth}|
    >{\centering\arraybackslash}p{0.2\textwidth}|
    >{\centering\arraybackslash}p{0.2\textwidth}@{}
}
\toprule
\textbf{Region} & \textbf{Publishing Date} & \textbf{Launching Date} & \textbf{Regulation Name} & \textbf{Article Reference} & \textbf{Operationalized Requirements} \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{C0C0C0}\textit{General Privacy Regulations}} \\ \midrule
 &  &  &  & Art.13.1.(a) & Controller Information \\
 &  &  &  & Art.13.2.(a) \& Art.14.2.(a) & Data Retention \\
 &  &  &  & Art.13.2.(b) \& 14.2.(c) & Right to Access \\
 &  &  &  & Art.13.2.(d) \& 14.2.(e) & Right to Lodge Complaints \\
 &  &  &  & Art.13.2.(c) \& 14.2.(d) & Right to be Forgotten \\
\multirow{-6}{*}{EU} & \multirow{-6}{*}{14-Apr-16} & \multirow{-6}{*}{25-May-18} & \multirow{-6}{*}{General Data Protection Regulation (GDPR)} & Art.13.2.(e) & Right to Lodge Complaints \\ \midrule
 &  &  &  & Art.15 & Right to be Forgotten \\
 &  &  &  & Art.17.(1) \& Art.52 & Controller Information \\
 &  &  &  & Art.17.(2) \& Art.19 & Data Retention \\
 &  &  &  & Art.31 & Protection of Minors \\
 &  &  &  & Art.45 & Right to Access \\
 &  &  &  & Art.50 & Right to Lodge Complaints \\
 &  &  &  & Art.51 & Risk Notification \\
\multirow{-8}{*}{China} & \multirow{-8}{*}{20-Aug-21} & \multirow{-8}{*}{1-Nov-21} & \multirow{-8}{*}{Personal Information Protection Act (PIPL)} & Art.51.(3) & Data Encryption \\ \midrule
 &  &  &  & Art.1798.120 & Right to be Forgotten \\
 &  &  &  & Art.1798.110 & Right to Access \\
\multirow{-3}{*}{California} & \multirow{-3}{*}{28-Jun-18} & \multirow{-3}{*}{1-Jan-20} & \multirow{-3}{*}{Consumer Privacy Act (CCPA)} & Art.1798.100.a.(3) & Data Retention \\ \midrule
 &  &  &  & Art.59.1-577.A.(1) & Right to Access \\
 &  &  &  & Art.59.1-577.A.(5) \& Art.59.1-578.(D) & Right to be Forgotten \\
 &  &  &  & Art.Art.59.1-577.(C) & Right to Lodge Complaints \\
\multirow{-4}{*}{Virginia} & \multirow{-4}{*}{2-Mar-21} & \multirow{-4}{*}{1-Jan-23} & \multirow{-4}{*}{Consumer Data Protection Act (CDPA)} & Art.59.1-579.A.(2) & Risk Notification \\ \midrule
\multicolumn{6}{c}{\cellcolor[HTML]{C0C0C0}\textit{GAI-specific Regulations}} \\ \midrule
 &  &  &  & Art.6.(b).1 \& Art.7.(f).1 \& Art.6.(b).2 & Prompt Guardrail \\
 &  &  &  & Art.5.2.(b).3 \& Art.7.(e) & Right to Lodge Complaints \\
 &  &  &  & Art.5.2.(b).4 \& Art.6.(b).2 & Risk Notification \\
 &  &  &  & Art.6.(a) \& Art.6.(c).1 \& Art.6.(c).2 & Base Model \\
 &  &  &  & Art.6.(c).1 & Target Users \\
 &  &  &  & Art.6.(c).1 & Tool Type \\
 &  &  &  & Art.7.(a).3 \& Art.7.(a).4 & Protection of Minors \\
 &  &  &  & Art.7.(c) & Right to be Forgotten \\
 &  &  &  & Art.7.(d) & AI-generated Watermarking \\
\multirow{-10}{*}{China} & \multirow{-10}{*}{11-Oct-23} & \multirow{-10}{*}{TBD} & \multirow{-10}{*}{\begin{tabular}[c]{@{}c@{}}Basic security requirements for \\ generative artificial intelligence service\end{tabular}} & Art.8.(a) & Third-party Audits \\ \midrule
 &  &  &  & Art.3.(b) & Base Model \\
 &  &  &  & Art.3.(d) \& Art.3 & Prompt Guardrail \\
 &  &  &  & Art.3.(e) \& Art.6.(a) & Risk Notification \\
 &  &  &  & Art.3.(f) & Tool Type \\
 &  &  &  & Art.3.(d) \& Art.3.(g) & Tool's Working Details \\
 &  &  &  & Art.5 & Third-party Audits \\
\multirow{-7}{*}{Singapore} & \multirow{-7}{*}{16-Jan-24} & \multirow{-7}{*}{TBD} & \multirow{-7}{*}{\begin{tabular}[c]{@{}c@{}}Model AI Governance Framework\\ for Generative AI\end{tabular}} & Art.7 & AI-generated Watermarking \\ \midrule
 &  &  &  & Art.3 & Data Encryption \\
 &  &  &  & Art.4 & AI-generated Watermarking \\
 &  &  &  & Art.4 & Risk Notification \\
 &  &  &  & Art.4 & Tool Type \\
 &  &  &  & Art.5 & Tool's Working Details \\
 &  &  &  & Art.6 & Right to Access \\
 &  &  &  & Art.7 & Data Retention \\
\multirow{-8}{*}{Canada} & \multirow{-8}{*}{7-Dec-23} & \multirow{-8}{*}{7-Dec-23} & \multirow{-8}{*}{\begin{tabular}[c]{@{}c@{}}Principles for responsible, trustworthy and\\ privacy-protective generative AI technologies\end{tabular}} & Art.8 & Prompt Guardrail \\ \midrule
EU &  & TBD & Artificial Intelligence Act (EU AI Act) & Art. 52 & AI-generated Watermarking \\ \midrule
 &  &  &  & Art.7 & Base Model \\
 &  &  &  & Art.10 & Target Users \\
 &  &  &  & Art.10 & Tool Type \\
 &  &  &  & Art.10 & Protection of Minors \\
 &  &  &  & Art.11 & Data Retention \\
 &  &  &  & Art.12 & AI-generated Watermarking \\
 &  &  &  & Art.14 & Risk Notification \\
\multirow{-8}{*}{China} & \multirow{-8}{*}{23-May-23} & \multirow{-8}{*}{15-Aug-23} & \multirow{-8}{*}{\begin{tabular}[c]{@{}c@{}}Administrative Measures for Generative\\ Artificial Intelligence Services\end{tabular}} & Art.15 \& Art.18 & Right to Lodge Complaints \\ \bottomrule
\end{tabular}
\caption{Regulations empirical study}
\end{table*}

==> table/user_study1.tex <==
\begin{table}[h]
\caption{Mean, Median, and SD for the eight statements}
\centering
\begin{tabular}{ccccc}
\toprule
\textbf{No.} & \textbf{Usability Aspect} & \textbf{Mean} & \textbf{Mdn} & \textbf{SD} \\ \midrule
$Q_1$ & User Needs & 3.98 & 4 & 1.11 \\
$Q_2$ & Reading Burden & 4.02 & 4 & 1.11 \\
$Q_3$ & Privacy Assurance & 4.08 & 4.5 & 1.20 \\
$Q_4$ & Trackability & 4.21 & 5 & 1.12 \\
$Q_5$ & Understandability & 4.06 & 4 & 1.03 \\
$Q_6$ & Interpretability & 4.31 & 5 & 0.98 \\
$Q_7$ & Concise Representation & 4.33 & 5 & 1.12 \\
$Q_8$ & Appropriate Volume & 4.5 & 5 & 0.89 \\ \bottomrule
\end{tabular}

\label{table:user study1}
\end{table}
